LM2D: Lyrics- and Music-Driven Dance Synthesis

Dance typically involves professional choreography with complex movements that follow a musical rhythm and can also be influenced by lyrical content. The integration of lyrics in addition to the auditory dimension, enriches the foundational tone and makes motion generation more amenable to its semantic meanings. However, existing dance synthesis methods tend to model motions only conditioned on audio signals. In this work, we make two contributions to bridge this gap. First, we propose LM2D, a novel probabilistic architecture that incorporates a multimodal diffusion model with consistency distillation, designed to create dance conditioned on both music and lyrics in one diffusion generation step. Second, we introduce the first 3D dance-motion dataset that encompasses both music and lyrics, obtained with pose estimation technologies. We evaluate our model against music-only baseline models with objective metrics and human evaluations, including dancers and choreographers. The results demonstrate LM2D is able to produce realistic and diverse dance matching both lyrics and music. A video summary can be accessed at: https://youtu.be/4XCgvYookvA.

==> draft.tex <==
% ==========
% 3D dance datasets play an essential role in the data-driven dance synthesis process. Unlike the 3D motion dataset, the 3D dance dataset usually requires much more professional experience and contains multi-modal information. 
% Motion capture techniques are widely used in 3D dance dataset construction. 
% \cite{alemi2017groovenet} released the first available 3D dance dataset with synchronized music using motion capture data. Electronic dance musics were selected and dancer's movements were captured using Vicon optical motion capture system, in total, 23 minutes of motion capture data. 
% Music2Dance~\cite{zhuang2022music2dance} collected synchronized music and motion capture of \textit{modern dance} and \textit{curtilage dance } for 58 minutes. 
% Later, In~\cite{valle2021transflower}, three new dance datasets, the popular music and street dance (PMSD) dataset, Syrtos dataset, and ShaderMotion VR dance dataset were introduced. 
% The PMSD dataset consists of 230.2 minutes of synchronized audio and motion capture recordings of various dancers and dance styles, including \textit{casual}, \textit{krump}, \textit{Hip-Hop}, and \textit{pop} dance. 
% The Syrtos dataset consists of 49.7 minutes of synchronized audio and motion capture recording of a specific Greek dance style - the \textit{Cretan Sytros}. 
% As the number of VR users grows, The ShaderMotion VR dance dataset introduces a new way to collect motion data from remote VR user participants. This data consists of 10.22 hours of motion, which was recorded by participants who danced on a social VR platform, VRChat. 
% Recently, ~\cite{alexanderson2023listen} combined a subset of the highest-quality recordings from the PMSD dataset with an additional dataset from three dancers in the genres \textit{Jazz}, \textit{Charleston}, \textit{Tap dancing}, and \textit{Locking}, yielding 373 minutes of parallel music audio and dance motion capture. 
% \cite{le2023music} and \cite{wang2022groupdancer} introduce music-driven group dance datasets, MCD and AIOZ-GDANCE dataset, totaling 1 hour and 16.7 hours, respectively. 
% DanceFormer~\cite{li2022danceformer} introduces the PhantomDance dataset, a 5-hour animated dance dataset, the first dance dataset created by professional animators.
% % ChoreoMaster~\cite{chen2021choreomaster} introduced a synchronized music and dance phrase dataset from both mocap resources and anime community resources.
% With the advance in 3D reconstruction methods, 3D dance data can be produced from 2D videos. \cite{li2021ai} use the AIST dance dataset~\cite{tsuchida2019aist} to obtain 3D dance motion using multi-view 3D pose estimation. 
% \cite{li2020learning} collected large amounts of high-quality videos from various dance channels on Youtube, and extracted 3D pose sequences with synchronized audios by VideoPose3d~\cite{pavllo20193d} 
% However, the currently available 3D dance dataset all aim to deal with music-driven dance synthesis, and hardly consider the influence of lyrics, which can add depth and enrich semantic meaning, as there is a notable connection between dance and song lyrics in styles like modern dance \cite{powell2019modern}. 
% To our knowledge, no dataset of synchronized music, lyrics, and body motion is currently available online. 
% \cite{lee2019talking} introduce a conversation dataset of audio, text, and motion modalities.
% To fill this gap, we construct a 3D dance dataset by 3D pose estimation to recover the dance sequence. We extracted the 3D pose sequences with synchronized audio and lyrics in total 4.6 hours. 


has been widely adopted for various applications, such as gesture generation, locomotion generation, motion style transfer, and dance generation. 



To enhance the understanding of our framework's effectiveness, we expanded our assessment approach beyond objective measures by conducting a user study. This study focused on evaluating three key aspects: the naturalness of motion, the alignment of motion with music, and the congruence of motion with lyrics. We engaged 30 dance-experienced individuals, whose expertise spanned areas like training, choreography, teaching, and performance. These participants had an average of 6.72 years of dance experience, with 23% (7 participants) possessing choreographic experience.

The study involved an online survey aimed at assessing the effectiveness of our lyrics and music-driven dance synthesis approach, collecting feedback through participant responses. We crafted 6-second video clips, juxtaposing ground truth footage with synthesized motion sequences. The presentation of these dance clips to participants was accompanied by questions. To mitigate any biases due to the sequence of clips, we ensured a random and balanced presentation order.

The evaluation was divided into two parts. The first part assessed motion naturalness and motion-music alignment, utilizing dance clips generated by LM2D, EDGE, LM2D-cd, EDGE-cd, or Ground Truth (GT). Participants had the option to review the clips multiple times before responding to the following two questions:

Motion Naturalness: "How much do you agree with the statement: 'The movements are natural and of high quality'?" - rated on a Likert scale from 1 (strongly disagree) to 5 (strongly agree).
Motion-Music Alignment: "How much do you agree with the statement: 'The movements synchronize well with the music's beat'?" - rated on a Likert scale from 1 (strongly disagree) to 5 (strongly agree).
The second part of the study focused on evaluating motion-lyrics matching. For this, dance clips generated by either LM2D or Ground Truth were used. Participants again had the opportunity to view these clips multiple times before answering:

Motion-Lyrics Matching: "How much do you agree with the statement: 'The movements harmonize well with the lyrics'?" - rated on a Likert scale from 1 (strongly disagree) to 5 (strongly agree).



% Figure \ref{fig: u1} indicates the performance of motion naturalness and motion-music alignment.
% 通过图片，我们可以观察到 在这两个指标上，我们发现参与者认为EDGE和LM2D于GT表现类似。而加了cd后的模型在效果上会略微下降。这与objective的发现类似。我们使用方差分析（ANOVA）来检验样本之间是否存在显著差异。
% 在motion naturalness上，在GT与EDGE和LM2D这三组中，根据方差分析（ANOVA）的结果，F统计量的值为0.0191，对应的p值为0.981。这个p值远高于常用的显著性水平（例如0.05），这表明这三组数据之间没有显著的差异。而在motion-music alignment上，方差分析（ANOVA）后，F统计量的值为0.1134，对应的p值为0.8929。这个p值远高于常用的显著性水平（例如0.05），这表明这三组数据之间没有显著的差异。
% 由此说明了我们的模型在加入了歌词的内容之后，在提升动作的丰富程度和语义内容的同时，还能保持动作的自然以及与音乐节拍的符合程度。

% 而在GT与EDGE-cd和LM2D这三组中，针对motion naturalness, 方差分析（ANOVA）后，F统计量的值为5.2529，对应的p值为0.0061。这个p值小于常用的显著性水平（例如0.05），这表明这三组数据之间存在显著的差异。
% 在motion-music alignment上，方差分析（ANOVA）后，F统计量的值为12.1948，对应的p值为1.0923e-05。这个p值远低于常用的显著性水平（例如0.05），这表明这三组数据之间存在显著的差异。这与表1的结果相符合，虽然在dance motion generation的过程中使用consistency distillation提高了效率，但是无论从客观指标还是human evaluation上来说 生成的效果都下降了，这也是在future work中需要提高的地方。

% Figure \ref{fig: u2} 中，我们着重比较了LM2D模型与ground truth之间的motion-lyrics matching。我们可以从图片中观察到，dance experts认为ground truth更符合。
% We use the two one-sided tests to determine if the means of the two systems evaluations are equivalent. 
% The equivalence margin was set at $\delta=0.05$. 结合两个单边检验的p值为0.799，高于通常用于表示统计显著性的阈值（如0.05
% 这意味着没有充分的证据支持两组数据在预定的等价区间内（本例中假设为±1）是等价的.
% 这表明了没有足够的证据表明这两组数据在统计学上是等价的。

